Fast and Modular Whole-Body Lagrangian Dynamics of Legged Robots with Changing Morphology

Fast and modular modeling of multi-legged robots (MLRs) is essential for resilient control, particularly under significant morphological changes caused by mechanical damage. Conventional fixed-structure models, often developed with simplifying assumptions for nominal gaits, lack the flexibility to adapt to such scenarios. To address this, we propose a fast modular whole-body modeling framework using Boltzmann-Hamel equations and screw theory, in which each leg's dynamics is modeled independently and assembled based on the current robot morphology. This singularity-free, closed-form formulation enables efficient design of model-based controllers and damage identification algorithms. Its modularity allows autonomous adaptation to various damage configurations without manual re-derivation or retraining of neural networks. We validate the proposed framework using a custom simulation engine that integrates contact dynamics, a gait generator, and local leg control. Comparative simulations against hardware tests on a hexapod robot with multiple leg damage confirm the model's accuracy and adaptability. Additionally, runtime analyses reveal that the proposed model is approximately three times faster than real-time, making it suitable for real-time applications in damage identification and recovery.

==> TRASHFILE.tex <==
% Maybe remove this paragraph (INTRO)
% Despite the significant research on this field, only a limited number of studies have actually modelled the dynamics of soft continuum systems. The constant curvature models had been limited to quasi-static motion at most to maintain accurate results and so have seen limited success capturing dynamics. Cosserat models were initially implemented for similar static or quasi-static applications but have the potential to capture system dynamics. Applications implementing this have been studied and validated with experimental results.\par


% COSSERAT ROD EQUATION DERIVATION WITH VARIATION APPLIED ON THE LAGRANGIAN
% The kinetic energy $KE$ of the continuum can be defined in terms of local velocity twists, $\eta$, and the Mass matrix as shown in \eqref{eq:KineticEnergy}. The internal energy $\mathcal{V}_{int}$ of the continuum can be defined in terms of the local strain twists, $\epsilon$, and the stiffness matrix as shown in \eqref{eq:InternalEnergy}. The external work done on the system $\mathcal{V}_{ext}$ by an applied load $g_{ext}$, which includes forces and moments in the local frame, i.e., wrenches, is shown in \eqref{eq:ExternalWork}. These energies of the system can be used to define the Lagrangian \eqref{eq:Lagrangian}.

% The kinetic energy, $KE$, and the internal energy, $\mathcal{V}_{int}$, of the continuum can be defined using the local mass and stiffness matrices as shown in \eqref{eq:KineticEnergy}\eqref{eq:InternalEnergy}. These energies of the system along with external work, defined as $\mathcal{V}_{ext}$, can be used to define the system Lagrangian \eqref{eq:Lagrangian}.

% \begin{align}
%     KE = \frac{1}{2} \displaystyle \int_L \eta ^T \textbf{M}\eta~ds \label{eq:KineticEnergy},\\
%     \displaystyle \mathcal{V}_{int} = \frac{1}{2} \int_L \epsilon^T\textbf{K}\epsilon~ds \label{eq:InternalEnergy},\\
%     %\displaystyle \mathcal{V}_{ext} = \int_L q^T g_{ext}~ds \label{eq:ExternalWork}\\
%     \displaystyle \mathcal{L} = KE - \mathcal{V}_{int} + \mathcal{V}_{ext} \label{eq:Lagrangian}.
% \end{align} 

% The Hamiltonian Principle can be applied as shown in  \eqref{eq:Hamilton} and results in the dynamic equation as shown in \eqref{eq:HamiltonPrinciple}. The variation of the different energies will be evaluated independently and the results combined to express the dynamics of the system. 
% \begin{gather}
%     \displaystyle \delta \int_{t_0}^{t_1} \mathcal{L}~dt = 0  \label{eq:Hamilton}, \\
%     \displaystyle \int_{t_0}^{t_1} (\delta(KE) - \delta(\mathcal{V}_{int}) + \delta(\mathcal{V}_{ext}))~dt = 0 \label{eq:HamiltonPrinciple}.
% \end{gather}

% % I DONT THINK THE DERIVATION OF VARIATIONS IS NECESSARY. WE CAN SHOW THE DIFFERENT TERMS THAT SHOW UP IN HAMILTONIAN AND CAN ADD A PARAGRAPH SAYING WHICH TERMS COME FROM WHICH IN THE FINAL DYNAMICAL EQUATION. JUST REFER TO GRAZIOSO FOR THE DERIVATION TO KEEP CONCISE
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The variation on the Kinetic Energy is derived as follows based on the variation of the velocity twists, the commutative property of Lie derivatives and the use of integration by parts. $\delta h$ is a twist $\in \se^\vee$ defined to have the following relation to the variation on the transformation, $H$, from the global into local frame: $\delta \big(H(t,s)\big) = H (\delta h)^\wedge$.
% %% WHAT IS THIS \delta h ??????????
% \begin{gather*}
%     \delta (KE) = {\displaystyle \int_L \delta(\eta) ^T \textbf{M}\eta~ds},\\
%     \delta(\eta) = \dot{(\delta h)} + \ad_{\eta}~\delta h,\\
%     \displaystyle \int_{t_0}^{t_1}(\delta(KE))~dt= \bigg[ \int_L \delta h^T \textbf{M}\eta~ds \bigg]_{t_0}^{t_1} - \\
%     \int_{t_0}^{t_1} \int_L \delta h^T (\textbf{M}\dot{\eta}-\ad_{\eta}^T\textbf{M}\eta)~ds~dt.
% \end{gather*}

% Similarly for the variation on the internal energy the following relations have also been derived similarly. The external load $g_{ext}$ is the applied force and moment, i.e., wrench, on the body expressed in the local frame.
% \begin{gather*}
%     \delta(\mathcal{V}_{int}) = \int_L \delta(\epsilon)^T\sigma ~ds,\\
%     \delta(\epsilon) = \delta(f) = (\delta h)'+\ad_{f}\delta h,\\
%     \displaystyle  \delta(\mathcal{V}_{int}) = \left[ \delta h^T \sigma \right]_0^L - \int_L \delta h^T (\sigma'-\ad_{f}^T\sigma)~ds,\\
%     \displaystyle  \delta(\mathcal{V}_{ext}) = \left[ \delta h^T g_{ext} \right]_0^L - \int_L \delta h^T g_{ext}~ds.
% \end{gather*}

% The strong form of these equations are obtained by combining the integrands of the 3 terms as these relations must be valid over arbitrary $\delta h$. This results in the following PDE to describe the dynamics of the system. The compatibility equation, to ensure the spatial and time derivatives are consistent, is also shown below derived from the definition of the $\ad$ operator \eqref{eq:adDef}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% BDF-2 ADJOINT MODIFICATION TO LOCAL FRAME 
% Note this general form for implicit discretization is expressed in global coordinates, as it does not adjust for changing coordinates when adding values at different time steps. Under the Lie Group framework, the strains and velocities are all defined in the local frames and hence cannot be added meaningfully without transforming values to the same coordinate. The following modification needs to be made to capture this change in coordinate frames for the local values used from previous time steps:

% \begin{gather*}
%     \dot{x}_i = c_0 x_i~+ \\
%     \Ad_{H_{Rot,i}}^{-1}~ \sum\limits_{k=1}^N \Ad_{H_{Rot,i-k}} \left[ c_k x_{i-k} + d_k \dot{x}_{i-k} \right],
% \end{gather*}
% \begin{align}
%     H_{Rot}= 
%     \begin{bmatrix}
%     H_{rot,3\times3} & 0_{3\times1}\\
%     0_{1\times3} & 1
%     \end{bmatrix} \label{eq:Hrot}.
% \end{align}

% $H_{Rot}$ is the transformation from the global to the local coordinate frame, but with the position component removed \eqref{eq:Hrot}. This transformation only causes a rotation of the twists from local to global coordinates but still expressed in the local frame.\par

% The previous values are known constants when solving for the approximation at a particular time step so these two components can be isolated when solving for the Boundary Condition (BC). Only the current value will then be iterated to satisfy the BC's. The implementation in this paper uses BDF-2 which is a second order approximation of the time derivative. The approximation using this discretization is as shown in \eqref{eq:BDF2Str}, and then \eqref{eq:BDF2Vel} after modified to be implemented on the Lie Group framework:

% \begin{gather}
%     \dot{f}_i = \frac{1}{\delta t}\left( 1.5 f_i - 2 f_{i-1} + 0.5 f_{i-2}\right) \label{eq:BDF2Str},\\
%     \dot{\eta}_i = \frac{1}{\delta t}\left( 1.5 \eta_i - \frac{2 \Ad_{H_{Rot,i-1}}} {\Ad_{H_{Rot,i}}} \eta_{i-1} + \frac{\Ad_{H_{Rot,i-2}}} {2 \Ad_{H_{Rot,i}}} \eta_{i-2}\right) \label{eq:BDF2Vel}.
% \end{gather}

% The modified time discretization is used to replace the time derivative of velocity but not the strain twists. The strain twists are discretized in the local coordinates directly. The strains come from the local stress-strain relations, which are only dependent on the local coordinates regardless of any change in the global frame. The velocity twists are discretized in global coordinates as the velocity do not depend on a local relation to define its response. Substituting these new expression as shown in \eqref{eq:BDF2Str} \eqref{eq:BDF2Vel}, then turns the set of PDE's into a set of ODE's in the spatial dimension. This is computationally cheaper to solve but comes at the price of a reduced accuracy solution compared to solving the original PDE's.



% JACOBIAN BC SOLVER
% It incorporates the state coupling through the use of a Jacobian to relate the change in the internal states at the end of the member to the change of internal states at its beginning. This Jacobian is numerically computed by perturbing the initial guess BC's independently to determine each of their effects on the end states by integrating the ODE dynamic equations.

% \begin{gather}
%     J_{i,j} = \frac{\delta f_{end,perturbed,j}}{\delta f_{base,perturbed,i}}\\
%     f_{base,new} = f_{base,old} + J^{-1} f_{end,old}
% \end{gather}

% The BC solver is given an iteration limit as well as a tolerance limit to terminate the solver when it finds a adequate solution or takes too long. Solver has been able to converge to solutions within reasonable tolerance for both static and dynamic cases, but can be improved by adapting solver parameters in Jacobian computations to introduce numerical damping to stabilize response and other adaptive features. \par


% EULER AND EXMP INTEGRATION
% The definition of the BC's complicate the solution process as they are not all known at the same location. The solution cannot be simply integrated using the ODE from the fixed end to the free end of the beam due to this issue, and so a BC solver using the Jacobian as described earlier was implemented to obtain all of the conditions at the start. \par
% % Idk if we need to talk about the euler integration thing at all
% Two Integration methods were tested and yielded similar results. They are Euler integration and exponential mapping on Lie Groups. The exponential mapping preserves the rotation matrix in the transformation, whereas the Euler integration does not without additional parameterization. The transformation propagation for the two methods are as shown below as they are integrated over s. Note the transformation is expressed in global coordinates for the location and orientation at reference length s with respect to the origin.
% 
% With the problem and solution method defined, the parameters and results of the simulation can now be addressed. The simulated problem geometry and BC were chosen to mimic Till's simulation so that the results can be compared. The parameters were also chosen, as shown in Table \ref{tab:Simulation_Variables}, to be identical in order to compare solution metrics, speed \& accuracy, between the classical and the Lie Group formulation.
